DiskANN++: Efficient Page-based Search over Isomorphic Mapped Graph Index using Query-sensitivity Entry Vertex

Given a vector dataset $\mathcal{X}$ and a query vector $\vec{x}_q$, graph-based Approximate Nearest Neighbor Search (ANNS) aims to build a graph index $G$ and approximately return vectors with minimum distances to $\vec{x}_q$ by searching over $G$. The main drawback of graph-based ANNS is that a graph index would be too large to fit into the memory especially for a large-scale $\mathcal{X}$. To solve this, a Product Quantization (PQ)-based hybrid method called DiskANN is proposed to store a low-dimensional PQ index in memory and retain a graph index in SSD, thus reducing memory overhead while ensuring a high search accuracy. However, it suffers from two I/O issues that significantly affect the overall efficiency: (1) long routing path from an entry vertex to the query's neighborhood that results in large number of I/O requests and (2) redundant I/O requests during the routing process. We propose an optimized DiskANN++ to overcome above issues. Specifically, for the first issue, we present a query-sensitive entry vertex selection strategy to replace DiskANN's static graph-central entry vertex by a dynamically determined entry vertex that is close to the query. For the second I/O issue, we present an isomorphic mapping on DiskANN's graph index to optimize the SSD layout and propose an asynchronously optimized Pagesearch based on the optimized SSD layout as an alternative to DiskANN's beamsearch. Comprehensive experimental studies on eight real-world datasets demonstrate our DiskANN++'s superiority on efficiency. We achieve a notable 1.5 X to 2.2 X improvement on QPS compared to DiskANN, given the same accuracy constraint.

==> src/ablation.tex <==
\begin{table}[t]
  \small
  \setstretch{1}
      \caption{Ablation experiments in different datasets on three components: query-sensitive entry vertex (A), isomorphic mapper (B), and pagesearch (C).}
      \label{tab:ablation_res}
      \begin{adjustbox}{width=\linewidth}
      \renewcommand{\arraystretch}{1.2}
      \begin{tabular}{ccccccc}
        \multicolumn{1}{c||}{Dataset}    & \multicolumn{3}{c|}{Recall@100=85\%}                                                                            & \multicolumn{3}{c}{Recall@100=97\%}                                                           \\ \hline
        \multicolumn{1}{c||}{sift100M}   & \multicolumn{3}{c|}{DiskANN++}                                                                                & \multicolumn{3}{c}{DiskANN++}                                                               \\ \hline \hline
        \multicolumn{1}{c||}{components} & \multicolumn{1}{c|}{QPS}             & \multicolumn{1}{c|}{mean I/Os} & \multicolumn{1}{c|}{mean hops} & \multicolumn{1}{c|}{QPS}            & \multicolumn{1}{c|}{mean I/Os} & mean hops     \\ \hline
        \multicolumn{1}{c||}{-}          & \multicolumn{1}{c|}{946.42 (1.00x)}  & \multicolumn{1}{c|}{181.54}    & \multicolumn{1}{c|}{24.66}            & \multicolumn{1}{c|}{385.88 (1.00x)} & \multicolumn{1}{c|}{447.49}    & 57.61                \\ \hline
        \multicolumn{1}{c||}{A}          & \multicolumn{1}{c|}{1033.64 (1.09x)} & \multicolumn{1}{c|}{164.57}    & \multicolumn{1}{c|}{22.51}            & \multicolumn{1}{c|}{401.14 (1.04x)} & \multicolumn{1}{c|}{431.58}    & 55.62                \\ \hline
        \multicolumn{1}{c||}{B}          & \multicolumn{1}{c|}{959.8 (1.01x)}   & \multicolumn{1}{c|}{181.54}    & \multicolumn{1}{c|}{24.66}            & \multicolumn{1}{c|}{387.17 (1.00x)} & \multicolumn{1}{c|}{447.49}    & 57.61                \\ \hline
        \multicolumn{1}{c||}{C}          & \multicolumn{1}{c|}{1065.09 (1.13x)} & \multicolumn{1}{c|}{179.24}    & \multicolumn{1}{c|}{24.38}            & \multicolumn{1}{c|}{440.34 (1.14x)} & \multicolumn{1}{c|}{438.87}    & 56.6                 \\ \hline
        \multicolumn{1}{c||}{AB}         & \multicolumn{1}{c|}{1022.24 (1.08x)} & \multicolumn{1}{c|}{164.57}    & \multicolumn{1}{c|}{22.51}            & \multicolumn{1}{c|}{397.41 (1.03x)} & \multicolumn{1}{c|}{431.58}    & 55.62                \\ \hline
        \multicolumn{1}{c||}{AC}         & \multicolumn{1}{c|}{1152.38 (1.22x)} & \multicolumn{1}{c|}{163.79}    & \multicolumn{1}{c|}{22.41}            & \multicolumn{1}{c|}{447.22 (1.16x)} & \multicolumn{1}{c|}{425.35}    & 54.92                \\ \hline
        \multicolumn{1}{c||}{BC}         & \multicolumn{1}{c|}{1281.32 (1.35x)} & \multicolumn{1}{c|}{148.32}    & \multicolumn{1}{c|}{20.58}            & \multicolumn{1}{c|}{660.6 (1.71x)}  & \multicolumn{1}{c|}{291.85}    & 38.25                \\ \hline
        \multicolumn{1}{c||}{ABC}        & \multicolumn{1}{c|}{1412.35 (1.49x)} & \multicolumn{1}{c|}{133.41}    & \multicolumn{1}{c|}{18.72}            & \multicolumn{1}{c|}{691.88 (1.79x)} & \multicolumn{1}{c|}{278.65}    & 36.62                \\
        \multicolumn{1}{l}{}            & \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{} \\
        \multicolumn{1}{c||}{Dataset}    & \multicolumn{3}{c|}{Recall@100=85\%}                                                                            & \multicolumn{3}{c}{Recall@100=97\%}                                                           \\ \hline
        \multicolumn{1}{c||}{deep100M}   & \multicolumn{3}{c|}{DiskANN++}                                                                                & \multicolumn{3}{c}{DiskANN++}                                                               \\ \hline \hline
        \multicolumn{1}{c||}{components} & \multicolumn{1}{c|}{QPS}             & \multicolumn{1}{c|}{mean I/Os} & \multicolumn{1}{c|}{mean hops} & \multicolumn{1}{c|}{QPS}            & \multicolumn{1}{c|}{mean I/Os} & mean hops     \\ \hline
        \multicolumn{1}{c||}{-}          & \multicolumn{1}{c|}{945.69 (1.00x)}  & \multicolumn{1}{c|}{184.15}    & \multicolumn{1}{c|}{25.06}            & \multicolumn{1}{c|}{308.78 (1.00x)} & \multicolumn{1}{c|}{557.93}    & 71.42                \\ \hline
        \multicolumn{1}{c||}{A}          & \multicolumn{1}{c|}{1104.46 (1.17x)} & \multicolumn{1}{c|}{153.7}     & \multicolumn{1}{c|}{21.25}            & \multicolumn{1}{c|}{325.66 (1.05x)} & \multicolumn{1}{c|}{529.26}    & 67.91                \\ \hline
        \multicolumn{1}{c||}{B}          & \multicolumn{1}{c|}{928.85 (0.98x)}  & \multicolumn{1}{c|}{184.15}    & \multicolumn{1}{c|}{25.06}            & \multicolumn{1}{c|}{305.81 (0.99x)} & \multicolumn{1}{c|}{557.93}    & 71.42                \\ \hline
        \multicolumn{1}{c||}{C}          & \multicolumn{1}{c|}{1043.07 (1.10x)} & \multicolumn{1}{c|}{177.15}    & \multicolumn{1}{c|}{24.19}            & \multicolumn{1}{c|}{332.42 (1.08x)} & \multicolumn{1}{c|}{549.1}     & 70.37                \\ \hline
        \multicolumn{1}{c||}{AB}         & \multicolumn{1}{c|}{1096.92 (1.16x)} & \multicolumn{1}{c|}{153.7}     & \multicolumn{1}{c|}{21.25}            & \multicolumn{1}{c|}{324.25 (1.05x)} & \multicolumn{1}{c|}{529.26}    & 67.91                \\ \hline
        \multicolumn{1}{c||}{AC}         & \multicolumn{1}{c|}{1156.4 (1.22x)}  & \multicolumn{1}{c|}{153.66}    & \multicolumn{1}{c|}{21.23}            & \multicolumn{1}{c|}{340.15 (1.10x)} & \multicolumn{1}{c|}{528.33}    & 67.74                \\ \hline
        \multicolumn{1}{c||}{BC}         & \multicolumn{1}{c|}{1296.92 (1.37x)} & \multicolumn{1}{c|}{142.83}    & \multicolumn{1}{c|}{19.92}            & \multicolumn{1}{c|}{588.93 (1.91x)} & \multicolumn{1}{c|}{316.78}    & 41.42                \\ \hline
        \multicolumn{1}{c||}{ABC}        & \multicolumn{1}{c|}{1523.41 (1.61x)} & \multicolumn{1}{c|}{118.89}    & \multicolumn{1}{c|}{16.99}            & \multicolumn{1}{c|}{625.23 (2.02x)} & \multicolumn{1}{c|}{291.78}    & 38.28                \\
        \multicolumn{1}{l}{}            & \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{} \\
        \multicolumn{1}{c||}{Dataset}    & \multicolumn{3}{c|}{Recall@100=85\%}                                                                            & \multicolumn{3}{c}{Recall@100=97\%}                                                           \\ \hline
        \multicolumn{1}{c||}{turing100M} & \multicolumn{3}{c|}{DiskANN++}                                                                                & \multicolumn{3}{c}{DiskANN++}                                                               \\ \hline \hline
        \multicolumn{1}{c||}{components} & \multicolumn{1}{c|}{QPS}             & \multicolumn{1}{c|}{mean I/Os} & \multicolumn{1}{c|}{mean hops} & \multicolumn{1}{c|}{QPS}            & \multicolumn{1}{c|}{mean I/Os} & mean hops     \\ \hline
        \multicolumn{1}{c||}{-}          & \multicolumn{1}{c|}{866.13 (1.00x)}  & \multicolumn{1}{c|}{202.21}    & \multicolumn{1}{c|}{27.22}            & \multicolumn{1}{c|}{136.12 (1.00x)} & \multicolumn{1}{c|}{1244.34}   & 157.5                \\ \hline
        \multicolumn{1}{c||}{A}          & \multicolumn{1}{c|}{990.49 (1.14x)}  & \multicolumn{1}{c|}{174.84}    & \multicolumn{1}{c|}{23.79}            & \multicolumn{1}{c|}{140.21 (1.03x)} & \multicolumn{1}{c|}{1215.26}   & 153.81               \\ \hline
        \multicolumn{1}{c||}{B}          & \multicolumn{1}{c|}{855.86 (0.99x)}  & \multicolumn{1}{c|}{202.21}    & \multicolumn{1}{c|}{27.22}            & \multicolumn{1}{c|}{136.33 (1.00x)} & \multicolumn{1}{c|}{1244.34}   & 157.5                \\ \hline
        \multicolumn{1}{c||}{C}          & \multicolumn{1}{c|}{988.52 (1.14x)}  & \multicolumn{1}{c|}{189.56}    & \multicolumn{1}{c|}{25.57}            & \multicolumn{1}{c|}{153.48 (1.13x)} & \multicolumn{1}{c|}{1203.58}   & 152.33               \\ \hline
        \multicolumn{1}{c||}{AB}         & \multicolumn{1}{c|}{958.94 (1.11x)}  & \multicolumn{1}{c|}{174.84}    & \multicolumn{1}{c|}{23.79}            & \multicolumn{1}{c|}{139.33 (1.02x)} & \multicolumn{1}{c|}{1215.26}   & 153.81               \\ \hline
        \multicolumn{1}{c||}{AC}         & \multicolumn{1}{c|}{1066.85 (1.23x)} & \multicolumn{1}{c|}{173.12}    & \multicolumn{1}{c|}{23.58}            & \multicolumn{1}{c|}{155.43 (1.14x)} & \multicolumn{1}{c|}{1187.15}   & 150.33               \\ \hline
        \multicolumn{1}{c||}{BC}         & \multicolumn{1}{c|}{1228.52 (1.42x)} & \multicolumn{1}{c|}{152.59}    & \multicolumn{1}{c|}{21.07}            & \multicolumn{1}{c|}{259.17 (1.90x)} & \multicolumn{1}{c|}{714.63}    & 91.37                \\ \hline
        \multicolumn{1}{c||}{ABC}        & \multicolumn{1}{c|}{1363.68 (1.57x)} & \multicolumn{1}{c|}{131.89}    & \multicolumn{1}{c|}{18.54}            & \multicolumn{1}{c|}{265.95 (1.95x)} & \multicolumn{1}{c|}{694.09}    & 88.84               
        \end{tabular}
      \end{adjustbox}
\end{table}

==> src/alg_cachedpagesearch.tex <==
\begin{algorithm}
\setstretch{0.82}
\small
    \caption{PageSearch($G$, $\vec{x}_{q}$, $v_{e}$, $B$, $L_s$, $k$)}
    \label{alg:pagesearch}
    \LinesNumbered
    \SetNoFillComment
    \KwIn{graph index ${G}$, query $\vec{x}_{q}$, enterpoint $v_{e}$, beam size ${B}$, search width $L_s$, size $k$ of top-k}
    \KwOut{approximate nearest top-$k$ neighbors $\mathcal{R}$ to $\vec{x}_q$}
    $\mathcal{C} \leftarrow \{v_e\}$ \tcc*[r]{{\footnotesize candidate set initialized as $\{v_e\}$}}
    $\mathcal{R} \leftarrow \emptyset$ \tcc*[r]{{\footnotesize top-$k$ results initialized as empty}}
    $\mathcal{H} \leftarrow PageHeap()$ \tcc*[r]{{\footnotesize PageHeap initialized as empty}}
    \Do{$\mathcal{F}\neq\emptyset$}{
        $\mathcal{F} \leftarrow$ top-$B$ unvisited vertices from $C$ for expansion \;
        \tcp{\small prepare for SSD I/O requests: lines 6-12}
        $\mathcal{P} \leftarrow \emptyset$ \tcc*[r]{{\footnotesize page placeholders initialized as empty}}
        \For{$v_i \in \mathcal{F}$}{
            \If{$\mathcal{H}\textnormal{.check2ret}(v_i)\textnormal{ is none}$}{
                $P_j \leftarrow$ register read for page containing $b_{v_i}$ \;
                $\mathcal{P} \leftarrow \mathcal{P} \cup P_j$ \;
            }
        }
        \tcp{\small async SSD I/O requests: line 13}
        submit async read requests $\mathcal{P}$ from SSD \;
        $\mathcal{H}$.update() \;
        \tcp{\small async page expansion: lines 15-22}
        \While{$b_{v_i}=\langle \vec{x}_{v_i},N(v_i) \rangle \leftarrow$ $\mathcal{H}$.pop()\textnormal{ is not none}}{
            \If{$v_i$\textnormal{ is unvisited}}{
                NeighborExpansion($\vec{x}_{q}$, $b_{v_i},\mathcal{C},\mathcal{R},L_s,k$) \;
                \If{\textnormal{async read done}}{
                    break \;
                }
            }
        }
        wait for async read done \;
        \tcp{\small node expansion: lines 25-28}
        $\mathcal{H}$.cache($\mathcal{P}$) \;
        \For{\textnormal{unvisited }$v_i \in \mathcal{F}$}{
            $b_{v_i}=\langle \vec{x}_{v_i},N(v_i) \rangle \leftarrow$ $\mathcal{H}$.check2ret($v_i$) \;
            NeighborExpansion($\vec{x}_{q}$, $b_{v_i},\mathcal{C},\mathcal{R},L_s,k$) \;
        }
        return $\mathcal{R}$
    }
\end{algorithm}

==> src/ep_experiment.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% % full table
% \begin{table}[]
% \caption{relationship between growth radio of hops and recall@100 in different $N_{cluster}$ on DEEP100M dataset.}
% \label{tab:ep_hops}
% \small
% \begin{tabular}{|c|cccccccc|}
% \hline
% \multirow{3}{*}{$N_{cluster}$} & \multicolumn{8}{c|}{recall@100 on deep100M}                                                                                                                                                \\ \cline{2-9} 
%                             & \multicolumn{1}{c|}{78} & \multicolumn{1}{c|}{81} & \multicolumn{1}{c|}{84} & \multicolumn{1}{c|}{87} & \multicolumn{1}{c|}{90} & \multicolumn{1}{c|}{93} & \multicolumn{1}{c|}{96} & 99   \\ \cline{2-9} 
%                             & \multicolumn{8}{c|}{Hops Growth Radio}                                                                                                                                                     \\ \hline \hline
% 1                           & 0                       & 0                       & 0                       & 0                       & 0                       & 0                       & 0                       & 0    \\
% 2                           & 6\%                     & 5\%                     & 5\%                     & 5\%                     & 4\%                     & 3\%                     & 2\%                     & 1\%  \\
% 4                           & -1\%                    & -1\%                    & -1\%                    & -1\%                    & -1\%                    & -1\%                    & 0\%                     & 0\%  \\
% 8                           & -4\%                    & -3\%                    & -3\%                    & -3\%                    & -3\%                    & -2\%                    & -1\%                    & -1\% \\
% 16                          & -6\%                    & -6\%                    & -5\%                    & -5\%                    & -4\%                    & -4\%                    & -2\%                    & -1\% \\
% 32                          & -14\%                   & -14\%                   & -13\%                   & -11\%                   & -10\%                   & -8\%                    & -5\%                    & -2\% \\
% 64                          & -10\%                   & -10\%                   & -9\%                    & -8\%                    & -7\%                    & -6\%                    & -4\%                    & -2\% \\
% 128                         & -13\%                   & -12\%                   & -11\%                   & -10\%                   & -9\%                    & -7\%                    & -5\%                    & -2\% \\
% 256                         & -14\%                   & -14\%                   & -13\%                   & -11\%                   & -10\%                   & -8\%                    & -5\%                    & -2\% \\
% 512                         & -16\%                   & -15\%                   & -14\%                   & -13\%                   & -11\%                   & -9\%                    & -6\%                    & -3\% \\
% 1024                        & -16\%                   & -15\%                   & -14\%                   & -12\%                   & -11\%                   & -9\%                    & -6\%                    & -3\% \\
% 2048                        & -16\%                   & -15\%                   & -14\%                   & -13\%                   & -11\%                   & -9\%                    & -6\%                    & -3\% \\
% 4096                        & -18\%                   & -18\%                   & -16\%                   & -15\%                   & -13\%                   & -10\%                   & -7\%                    & -3\% \\
% 8192                        & -19\%                   & -18\%                   & -16\%                   & -15\%                   & -13\%                   & -11\%                   & -7\%                    & -3\% \\
% 16384                       & -19\%                   & -18\%                   & -17\%                   & -16\%                   & -13\%                   & -11\%                   & -7\%                    & -3\% \\
% 32768                       & -20\%                   & -19\%                   & -17\%                   & -16\%                   & -14\%                   & -11\%                   & -7\%                    & -3\% \\
% 65536                       & -20\%                   & -19\%                   & -17\%                   & -16\%                   & -14\%                   & -11\%                   & -7\%                    & -3\% \\ \hline
% \end{tabular}
% \end{table}

% % slim table
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \caption{relationship between growth radio of hops/QPS and recall@100 in different $N_{cluster}$ on deep100M dataset.}
% \label{tab:ep_hops_qps}
% \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{|c|cccccc|}
% \hline
% \multirow{3}{*}{N\_cluster} & \multicolumn{6}{c|}{recall@100 on deep100M}                                                                                              \\ \cline{2-7} 
%                             & \multicolumn{1}{c|}{87} & \multicolumn{1}{c|}{93} & \multicolumn{1}{c|}{99}   & \multicolumn{1}{c|}{87} & \multicolumn{1}{c|}{93} & 99   \\ \cline{2-7} 
%                             & \multicolumn{3}{c|}{Hops Growth Radio}                                        & \multicolumn{3}{c|}{QPS Growth Radio}                    \\ \hline \hline
% 1                           & 0                       & 0                       & \multicolumn{1}{c|}{0}    & 0                       & 0                       & 0    \\
% 2                           & 5\%                     & 3\%                     & \multicolumn{1}{c|}{1\%}  & -5\%                    & -4\%                    & -1\% \\
% 4                           & -1\%                    & -1\%                    & \multicolumn{1}{c|}{0\%}  & 1\%                     & 0\%                     & 0\%  \\
% 8                           & -3\%                    & -2\%                    & \multicolumn{1}{c|}{-1\%} & 4\%                     & 3\%                     & 1\%  \\
% 16                          & -5\%                    & -4\%                    & \multicolumn{1}{c|}{-1\%} & 6\%                     & 3\%                     & 1\%  \\
% 32                          & -11\%                   & -8\%                    & \multicolumn{1}{c|}{-2\%} & 15\%                    & 7\%                     & 2\%  \\
% 64                          & -8\%                    & -6\%                    & \multicolumn{1}{c|}{-2\%} & 10\%                    & 6\%                     & 2\%  \\
% 128                         & -10\%                   & -7\%                    & \multicolumn{1}{c|}{-2\%} & 12\%                    & 7\%                     & 2\%  \\
% 256                         & -11\%                   & -8\%                    & \multicolumn{1}{c|}{-2\%} & 15\%                    & 7\%                     & 2\%  \\
% 512                         & -13\%                   & -9\%                    & \multicolumn{1}{c|}{-3\%} & \textbf{16\%}           & 10\%                    & 3\%  \\
% 1024                        & -12\%                   & -9\%                    & \multicolumn{1}{c|}{-3\%} & 15\%                    & 9\%                     & 2\%  \\
% 2048                        & -13\%                   & -9\%                    & \multicolumn{1}{c|}{-3\%} & \textbf{16\%}           & 10\%                    & 2\%  \\
% 4096                        & -15\%                   & -10\%                   & \multicolumn{1}{c|}{-3\%} & 17\%                    & 10\%                    & 2\%  \\
% 8192                        & -15\%                   & -11\%                   & \multicolumn{1}{c|}{-3\%} & 15\%                    & 9\%                     & 2\%  \\
% 16384                       & \textbf{-16\%}          & -11\%                   & \multicolumn{1}{c|}{-3\%} & 12\%                    & 7\%                     & 1\%  \\
% 32768                       & \textbf{-16\%}          & -11\%                   & \multicolumn{1}{c|}{-3\%} & 7\%                     & 2\%                     & 1\%  \\
% 65536                       & \textbf{-16\%}          & -11\%                   & \multicolumn{1}{c|}{-3\%} & -7\%                    & -7\%                    & -3\% \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ncluster_vs_opt.pdf}
    \caption{Relationship between changing of hopcount/QPS and recall@100 in different $N_{cluster}$ on deep100M dataset, the larger the better.}
    \label{fig:ep_hops_qps}
\end{figure}

==> src/isotrans_theory.tex <==
% This section, we theoretically prove and calculate that the packing algorithm can stably improve the compactness of nodes within each disk page.
% [deleted] , and the merging algorithm can guarantee that each set has exactly the capacity of a page (i.e. linear).
% We quantitatively measure the compactness of nodes within a page by evaluating the diameter and algebraic connectivity of the subgraph derived from the nodes within the page.
In this section, we present a comprehensive theoretical analysis and calculation to demonstrate the efficacy of the packing algorithm. We substantiate that the algorithm reliably enhances the cohesiveness of nodes on individual disk pages. This is achieved through a quantitative assessment of node compactness within each page, which is based on an evaluation of both the subgraph's diameter and its algebraic connectivity, derived from the constituent nodes within the page.

For convenience, we will restate some mathematical definitions that will be used.

\begin{definition}[diameter of a graph]
    The diameter of graph \( \text{diam}(G(V,E)) \) is defined as
    \[
    \text{diam}(G(V,E)) = \max_{u, v \in V} \text{shortest\_path}(u, v)
    \]
    
    where $\text{shortest\_path}(u, v)$ represents the length of the shortest path between nodes $u$ and $v$.
\end{definition}

\begin{definition}[Laplacian matrix of a graph]
    Laplacian matrix $L(G)$ of graph $G(V,E)$ is defined as
    \[
    L_{i,j}(G)=
    \begin{cases}
        deg(v_i) & \text{if } i=j \\
        -1 & \text{if } i\neq j \text{ and } v_i \text{ is adjacent to } v_j \\
        0 & \text{otherwise}
    \end{cases}
    \]
    where $v_i, v_j\in V$. In the absence of dissent, $L(G)$ can be succinctly denoted as $L$ or $L_G$.
\end{definition}

\begin{definition}[algebraic connectivity of a graph]
    The algebraic connectivity of graph \( \lambda_2(G) \) is defined as the second-smallest eigenvalue (counting multiple eigenvalues separately) of the Laplacian matrix of the graph, i.e.
    \[
    \lambda_2(G) = \min_{\genfrac{}{}{0pt}{3}{x \perp \mathbf{1}}{x \neq \mathbf{0}}} \frac{x^T L x}{x^T x}
    \]
    where \( \mathbf{0}=(0,0,...,0)^t \), \( \mathbf{1}=(1,1,...,1)^t \). \( L  \) is Laplacian matrix of the corresponding graph. Additionally, we denote the eigenvalues of \(L\) in ascending order as \(\lambda_i, i=1,2,...\).
\end{definition}

\begin{definition}[star graph]
\label{def:star}
    A r-star consists of \(1\) central vertex and \(r-1 (r \geq 1)\) peripheral vertices connected to the central vertex, with no connections between the peripheral vertices. It can be represented as \( S_r \), e.g. \Cref{fig:star} refers to some common types of stars.
\end{definition}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3-star.pdf}
         \caption{$S_3$ - 3-star}
         \label{fig:3-star}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/4-star.pdf}
         \caption{$S_4$ - 4-star}
         \label{fig:4-star}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/5-star.pdf}
         \caption{$S_5$ - 5-star}
         \label{fig:5-star}
     \end{subfigure}
        \caption{Different types of stars, each star has \(1\) central vertex and \(r-1\) independent peripheral vertices connected to the central vertex}
        \label{fig:star}
\end{figure}

\begin{definition}[$a$-bounded star partition]
    A star partition of graph $G(V, E)$ is a partition of the node set $V$ into subsets ${V_0, V_1, ..., V_i}$ so that the subgraph induced by each subset has a spanning star. Particularly, when the cardinality of nodes within each subset is no greater than $a$, it is referred to as an $a$-bounded star partition. \Cref{fig:star_partition} is an example of available 4-bounded star partition to a graph.
\end{definition}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/star_partition.pdf}
  \caption{describes a $\mathbf{4}$-bounded star partition on the graph. The induced subgraph of nodes with the same color contains a $\mathbf{4}$-star or $\mathbf{3}$-star or $\mathbf{1}$-star.}
  \label{fig:star_partition}
\end{figure}

It is evident that the packing algorithm applies a $cap$-bounded star partition to the Vamana graph.

\begin{definition}[node compactness]
    The node compactness $\gamma$ of graph \(G\)  is defined as
    \begin{align}
        \gamma(G) &= ( diam^{-1}(G), \lambda_2(G) ) \nonumber \\
                    &= ( diam^{-1}, \lambda_2)(G) \nonumber
    \end{align}
\end{definition}

\begin{definition}[partial order relation of compactness]
    We define
    \begin{gather}
        \gamma(G)<\gamma(G') \nonumber \\ 
        \Leftrightarrow \nonumber \\
        \begin{cases}
            \lambda_2(G)<\lambda_2(G'), &  diam^{-1}(G)=diam^{-1}(G') \\
            diam^{-1}(G)<diam^{-1}(G'), & others \nonumber \\
        \end{cases}
    \end{gather}
    Thus, we can compare compactness of different graphs.
\end{definition}

The partial order relation of compactness dictates that graphs with smaller diameter are more tightly connected. Besides, when two graphs share the same diameter, those with better connectivity exhibit higher compactness. In particular, disconnected graphs have smallest compactness. Furthermore, due to the extensively explored algebraic properties of undirected graphs, and in order to streamline the issue at hand, we make the following approximations:

\begin{approximation}[random]
    \textnormal{Because of the random order of the vector data, which leads to the randomness of node indices, we approximate that the Vamana graph is a \textbf{random} R-regular graph. In subsequent discourse, this approximation is only employed for the computation of edge probabilities in the graph (see \Cref{lemma:edgePRB})}.
\end{approximation}

\begin{approximation}[undirected]
    \textnormal{It can be noticed that the Vamana index-building algorithm [\todo{citation:diskann}] leads to the retention of a significant number of reverse edges in the directed graph. It has been verified through experiments (see \todo{Figure: Edge Proportion}) across various situations, including different neighbor limit (\(R\)) and candidate set limit (\(Lc\)). In all cases, more than two-thirds of the edges have a corresponding reverse edge. Therefore, for the sake of analytical convenience, we approximate all edges in the Vamana graph as undirected edges, transforming Vamana into an \textbf{undirected} graph, which makes it possible to do Laplacian matrix analysis on the Vamana graph.}
\end{approximation}

\begin{lemma}
\label{lemma:edgePRB}
    In a random R-regular graph \(Gr\) with N nodes, the probability of an edge connecting two nodes \( p(v_i,v_j) \) is 
    \[ 
        p(<v_i,v_j> \in Gr)=\frac{R^2}{NR-1}, (R\ll N)
    \]
    \begin{proof}
        We employ a similar proof based on the configuration model [\todo{citation}]. 
        
        Considering each edge as 2 stubs, we explore the possibility of connecting a stub from \(v_i\) to any stub of \(v_j\). As the edges are uniformly distributed, this probability is given by \(R/(NR-1)\) (selecting R out of all stubs except its own). Since \(v_i\) has R independent stubs of this nature, the probability of there being an edge between node \(v_i\) and node \(v_j\) is \(R^2/(2NR-1)\).
    \end{proof}
\end{lemma}

\begin{proposition}
\label{proposition:isolated}
    In a random R-regular graph Gr with N nodes, if we select a node set of size c (where \(c\le R\ll N)\) consisting of nodes with consecutive indices, then the subgraph induced by this node set in graph Gr is almost not connected.
    \begin{proof}
        In the R-regular graph generated by the configuration model mentioned in \Cref{lemma:edgePRB}, the conclusion is apparent. Considering the probability that an arbitrary node \(w_i\) is isolated within the induced subgraph \(Gr_c\). Then
        \[
        \begin{aligned}
            p(w_i\text{ is isolated})
            &=\prod \limits_{i\neq j}{\{1-p(<w_i,w_j>\in G_r)\}} \\
            &=(1-\frac{R^2}{NR-1})^{c-1}
        \end{aligned}
        \]
        Since we have 
        \[
        w_i\text{ is isolated} \rightarrow Gr_c\text{ is not connected}
        \]
        then
        \begin{equation}
        \label{equ:squeeze}
        \begin{aligned}
        (1-\frac{R^2}{NR-1})^{c-1}&=p(w_i\text{ is isolated}) \\
        &\le p(Gr_c\text{ is not connected}) \\
        &\le 1
        \end{aligned}
        \end{equation}
        When \(R \ll N\), the \cref*{equ:squeeze} yields (Squeeze theorem)
        \[
        p(Gr_c\text{ is not connected})=1
        \]
    \end{proof}
\end{proposition}
    
\begin{proposition}
    \label{diskann_compactness}
    The node compactness of a random R-regular graph \(Gr\) with \(N\) nodes in size \(c\) page is \((0, 0)\).
    \begin{proof}
        Remark the induced subgraph of \(Gr\) with size \(c\) as \(Gr_c\). Firstly, \(diam^{-1}(Gr_c)=\frac{1}{\infty}=0\) since \(Gr_c\) is not connected derived from \Cref{proposition:isolated}. Secondly, without loss of generality, assume that \(Gr_c\) consists of two independent connected components \(G_1\) and \(G_2\). In this case, the Laplacian matrix \(L\) of \(Gr_c\) can be represented as
        \[
        L=
        \begin{bmatrix}
            L_{G_1} & \mathbf{0} \\
            \mathbf{0} & L_{G_2} \\
        \end{bmatrix}
        \]
        Obviously, we have 
        \[
        \begin{bmatrix}
            L_{G_1} & \mathbf{0} \\
            \mathbf{0} & L_{G_2} \\
        \end{bmatrix}
        \begin{bmatrix}
            \mathbf{1} \\
            \mathbf{0} \\
        \end{bmatrix}
        =
        \begin{bmatrix}
            L_{G_1} & \mathbf{0} \\
            \mathbf{0} & L_{G_2} \\
        \end{bmatrix}
        \begin{bmatrix}
            \mathbf{0} \\
            \mathbf{1} \\
        \end{bmatrix}
        =
        \begin{bmatrix}
            \mathbf{0} \\
            \mathbf{0} \\
        \end{bmatrix}
        \]
        Hence \(\alpha_1=(1,...,1,0,...,0)^T\) and \(\alpha_2=(0,...,0,1,...,1)^T\) are eigenvectors corresponding to eigenvalue \(\mathbf{0}\) of \(L\). On the other hand, \(L\) is symmetric and diagonally dominant, then \(0\leq \lambda_1\leq \lambda_2\leq \lambda_3\leq ...\). Hence we have \(\lambda_2(Gr_c)=0\).

        Therefore, \(\gamma(Gr_c)=(0,0)\)
    \end{proof}
\end{proposition}

\begin{lemma}
    \label{packing_compactness}
    The node compactness of a star \(S_k (k>1)\) \(\gamma(S_k)=(\frac{1}{2}, 1)\).
    \begin{proof}
        By \Cref{def:star}, we can obtain \(diam^{-1}(S_k)=\frac{1}{2}\). Additionally, we can employ spectral decomposition to the Laplacian matrix \(L\) of \(S_k\)
        \[
        L=
        \begin{bmatrix}
            k-1 & -\mathbf{1} \\
            -\mathbf{1} & \mathbf{E} \\
        \end{bmatrix}
        \]
        where \(\mathbf{E}\) is identity matrix.
        Hence we get the eigenvectors \( \xi \) with the corresponding eigenvalues \( \lambda \)
        \begin{gather}
        \lambda_i=
        \begin{cases}
        0, \xi=\mathbf{1}^T, & i=1 \\
        1, \xi=(0,a_2,a_3,...,a_k)^T, (\sum\limits_{p=2}^k{a_p}=1), & i=2,3,...,k-1 \\
        k, \xi=(1-k,1,1,..,1)^T, & i=k \\
        \end{cases}
        \end{gather}
        Since \(k>1\), then we get \(\lambda_2(S_k)=1\). Therefore, \(\gamma(S_k)=(\frac{1}{2}, 1)\).
    \end{proof}
\end{lemma}

\begin{proposition}
    Combining \Cref{diskann_compactness} and \Cref{packing_compactness}, we can derive the conclusion that the induced star graphs obtained through star partitioning on a random R-regular graph with \(N\) nodes always have higher node compactness (\( R\ll N \)).
\end{proposition}

Based on this, it can be concluded that \Cref{algorithm:packing} enables high speed star partitioning on graph and \Cref{algorithm:merging} maps the nodes within a star to the same disk page, thereby stably enhancing node compactness within disk pages.

\todo{provement for merging (bin-packing)}

==> src/neighbor_expand.tex <==
\begin{algorithm}[t]
\caption{NeighborExpansion($\vec{x}_{q}$, $b_v$, $\mathcal{C}$, $\mathcal{R}$, $L_s$, $k$)}
\label{alg:neighbor_expand}
\LinesNumbered
\SetNoFillComment
\KwIn{query $\vec{x}_{q}$, data block $b_v=\langle \vec{x}_v,N(v) \rangle$, PQ distance based ordered set $\mathcal{C}$, full distance based ordered set $\mathcal{R}$, search width $L_s$, size $k$ of top-k}
$\mathcal{C} \leftarrow \mathcal{C}\cup N(v)$ \tcc*[r]{{\footnotesize sort $\mathcal{C}$ by PQ distance to $\vec{x}_q$}}
\While{$|\mathcal{C}| > L_s$}{
    pop back from $\mathcal{C}$ \;
}
$\mathcal{R} \leftarrow \mathcal{R}\cup \{v\}$ \tcc*[r]{{\footnotesize sort $\mathcal{R}$ by full distance to $\vec{x}_q$}}
\While{$|\mathcal{R}| > k$}{
    pop back from $\mathcal{R}$ \;
}
\end{algorithm}

==> src/overhead_ep.tex <==
\begin{table}[t]
  \small
  \setstretch{0.75}
      \caption{The overhead and speedup (on recall@100=97\% in deep100M) of query-sensitive entry vertex pre-selection.}
      \label{tab:overhead_of_ep}
      \begin{adjustbox}{width=\linewidth}
      \renewcommand{\arraystretch}{1.2}
      \begin{tabular}{c||cc|cc|l}
        & \multicolumn{2}{c|}{DRAM}                & \multicolumn{2}{c|}{TIME}                 &                          \\ \hline \hline
entry vertex pre-selection   strategy & \multicolumn{1}{c|}{absolute} & relative & \multicolumn{1}{c|}{absolute}  & relative & speedup                  \\ \hline
linear scan                           & \multicolumn{1}{c|}{1.5MB}    & 0.04\%   & \multicolumn{1}{c|}{131.19 ms} & 0.64\%   & \multicolumn{1}{c}{12\%} \\ \hline
ANN graph search (faiss)              & \multicolumn{1}{c|}{1.7MB}    & 0.04\%   & \multicolumn{1}{c|}{8.55 ms}   & 0.04\%   & \multicolumn{1}{c}{12\%}
\end{tabular}
      \end{adjustbox}
  \end{table}

==> src/overhead_reorder.tex <==
\begin{table*}[t]
\centering
  %\setstretch{0.75}
  \caption{Overhead and speedup (at recall@100=97\%) of randomOrder, parallelGorder, pack-merge (ours) using pagesearch.}
  \label{tab:overhead_of_reorder}
  \scalebox{0.85}{
  \begin{adjustbox}{width=\linewidth}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{c||ccc|ccc|ccc}
                              & \multicolumn{3}{c|}{DRAM usage (GB)} & \multicolumn{3}{c|}{re-indexing time (s)} & \multicolumn{3}{c}{speedup with   pagesearch}\\ \hline \hline
      graph index             & \multicolumn{1}{c|}{randomOrder}     & \multicolumn{1}{c|}{parallelGorder}       & starPacking                                   & \multicolumn{1}{c|}{randomOrder} & \multicolumn{1}{c|}{parallelGorder} & starPacking & \multicolumn{1}{c|}{randomOrder} & \multicolumn{1}{c|}{parallelGorder} & starPacking \\ \hline
      Vamana (sift100M R32)   & \multicolumn{1}{c|}{2.2}             & \multicolumn{1}{c|}{75.1 (MLE)}           & 6.3                                           & \multicolumn{1}{c|}{449.5}       & \multicolumn{1}{c|}{2739.1}         & 222.3       & \multicolumn{1}{c|}{1.02x}       & \multicolumn{1}{c|}{1.84x}          & 1.69x       \\ \hline
      Vamana (deep100M R32)   & \multicolumn{1}{c|}{1.9}             & \multicolumn{1}{c|}{72.5 (MLE)}           & 5.1                                           & \multicolumn{1}{c|}{381.2}       & \multicolumn{1}{c|}{2651.4}         & 123.1       & \multicolumn{1}{c|}{1.08x}       & \multicolumn{1}{c|}{2.15x}          & 2.02x       \\ \hline
      Vamana (turing100M R32) & \multicolumn{1}{c|}{2.0}             & \multicolumn{1}{c|}{73.4 (MLE)}           & 6.1                                           & \multicolumn{1}{c|}{366.7}       & \multicolumn{1}{c|}{2644.8}         & 195.2       & \multicolumn{1}{c|}{1.08x}       & \multicolumn{1}{c|}{2.08x}          & 1.88x
    \end{tabular}
  \end{adjustbox}
  }
\end{table*}
